CamJ: Enabling System-Level Energy Modeling and Architectural Exploration for In-Sensor Visual Computing

CMOS Image Sensors (CIS) are fundamental to emerging visual computing applications. While conventional CIS are purely imaging devices for capturing images, increasingly CIS integrate processing capabilities such as Deep Neural Network (DNN). Computational CIS expand the architecture design space, but to date no comprehensive energy model exists. This paper proposes CamJ, a detailed energy modeling framework that provides a component-level energy breakdown for computational CIS and is validated against nine recent CIS chips. We use CamJ to demonstrate three use-cases that explore architectural trade-offs including computing in vs. off CIS, 2D vs. 3D-stacked CIS design, and analog vs. digital processing inside CIS. The code of CamJ is available at: https://github.com/horizon-research/CamJ

==> exp.tex <==
\section{Experimental Setup}


==> table/table_analog_functional_component.tex <==
\begin{table*}[t]
%\scriptsize

\centering
\caption{Supported Analog Functional Components}
\begin{tabular}{|cc|ccc|}
\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Analog Functional Component}}}                                                                                                   & \multicolumn{3}{c|}{\textbf{Analog Circuit Cell}}                       \\ \cline{3-5} 
\multicolumn{2}{|c|}{}                                                                                                                                                        & \multicolumn{1}{c|}{Dynamic} & \multicolumn{1}{c|}{Static} & Non-linear \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{APS pixel}}                                                          & PD                                                                & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}source\\ follower\end{tabular}         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{x}      &            \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{PWM pixel}}                                                          & PD                                                                & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}ramp\\ generator\end{tabular}          & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{x}      &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}dynamic\\ comparator\end{tabular}      & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{DPS pixel}}                                                          & PD                                                                & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & ADC                                                               & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}       & x          \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}passive\\ analog memory\end{tabular}}                     & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}active\\ analog memory\end{tabular}}}     & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}unity-gain\\ buffer\end{tabular}       & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{x}      &            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}current-domain\\ MAC\end{tabular}}}       & current mirror                                                    & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{x}      &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}charge-domain\\ passive MAC\end{tabular}}                 & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}charge-domain\\ active MAC\end{tabular}}} & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}switched-cap\\ integrator\end{tabular} & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{x}      &            \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}voltage-domain\\ max\end{tabular}}}       & \begin{tabular}[c]{@{}c@{}}common-source\\ amplifier\end{tabular} & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & current bias                                                      & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{x}      &            \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{log(x1/x2)}}\tianrui{scaling, absolute difference}                                                         & capacitor                                                         & \multicolumn{1}{c|}{x}       & \multicolumn{1}{c|}{}       &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & \begin{tabular}[c]{@{}c@{}}differential\\ OpAmp\end{tabular}      & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{x}      &            \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                                                                    & comparator                                                        & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}       & x          \\ \hline
\end{tabular}
\label{tbl:analog_functional_component}
\end{table*}

==> table/table_analog_hardware_interface.tex <==
\begin{table}[t]
%\scriptsize

\centering
\caption{Key analog hardware interface \fixme{update this.}}
\begin{tabular}{|cl|}
\hline
\multicolumn{2}{|c|}{\textbf{Analog Functional Array}}                                                                                                                                    \\ \hline
\multicolumn{1}{|c|}{position}             & \begin{tabular}[c]{@{}l@{}}array position:\\ \{'pixel', 'column', 'chip'\}\end{tabular}                                                      \\ \hline
\multicolumn{1}{|c|}{num\_input/output}    & \begin{tabular}[c]{@{}l@{}}\# input/output wires to/from the array\\ \textit{tuple, 2-D array for each data} type\end{tabular}                        \\ \hline
\multicolumn{1}{|c|}{num\_component}       & \begin{tabular}[c]{@{}l@{}}\# identical components in the array\\ \textit{2-D array}\end{tabular}                                                     \\ \hline
\multicolumn{2}{|c|}{\textbf{Analog Functional Component}}                                                                                                                                \\ \hline
\multicolumn{1}{|c|}{name}                 & component name                                                                                                                               \\ \hline
\multicolumn{1}{|c|}{num\_input/output}    & \begin{tabular}[c]{@{}l@{}}\# input/output wires to/from the component\\ \textit{tuple, 2-D array for each data type}\end{tabular}                    \\ \hline
\multicolumn{1}{|c|}{domain\_input/output} & \begin{tabular}[c]{@{}l@{}}input/output signal domain of the component:\\ \{'optical', 'voltage', 'charge', 'current', 'time'\}\end{tabular} \\ \hline
\multicolumn{1}{|c|}{delay}                & operation latency of the component                                                                                                           \\ \hline
\multicolumn{1}{|c|}{energy}               & energy consumption of the component                                                                                                          \\ \hline
\end{tabular}
\end{table}

==> table/table_usecase_gazetracking.tex <==
\begin{table}[t]
%\scriptsize

\centering
\caption{Energy Estimation of Analog and Digital Implementations For Gaze-Tracking CIS [pJ/pixel]}
\begin{tabular}{|ccc|cc|}
\hline
\multicolumn{3}{|c|}{\textbf{Domain}}                                                                                                                                  & \multicolumn{1}{c|}{Digital} & \begin{tabular}[c]{@{}c@{}}Analog (Stage 1+2)\\ +Digital\end{tabular} \\ \hline
\multicolumn{3}{|c|}{\textbf{Technology}}                                                                                                                              & \multicolumn{2}{c|}{110nm}                                                                           \\ \hline
\multicolumn{3}{|c|}{\textbf{Frame Rate}}                                                                                                                              & \multicolumn{2}{c|}{90fps}                                                                           \\ \hline
\multicolumn{1}{|c|}{\multirow{8}{*}{\textbf{Energy}}} & \multicolumn{2}{c|}{Pixel}                                                                                    & \multicolumn{1}{c|}{3.1}     & 3.2                                                                   \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{ADC}                                                                                      & \multicolumn{1}{c|}{22.8}    & -                                                                     \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Digital\\ Frame Buffer\end{tabular}}} & Access & \multicolumn{1}{c|}{199.4}   & \multirow{2}{*}{-}                                                    \\ \cline{3-4}
\multicolumn{1}{|c|}{}                                 & \multicolumn{1}{c|}{}                                                                                & Leakge & \multicolumn{1}{c|}{}        &                                                                       \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Analog\\ Frame Buffer\end{tabular}}                            & \multicolumn{1}{c|}{-}       & 12.1                                                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Digital PE}                                                                               & \multicolumn{1}{c|}{1.5}     & -                                                                     \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Analog PE}                                                                                & \multicolumn{1}{c|}{-}       & 24.4                                                                  \\ \cline{2-5} 
\multicolumn{1}{|c|}{}                                 & \multicolumn{2}{c|}{Output Buffer}                                                                            & \multicolumn{1}{c|}{}        & 1.02                                                                  \\ \hline
\multicolumn{3}{|c|}{\textbf{Power}}                                                                                                                                   & \multicolumn{1}{c|}{}        &                                                                       \\ \hline
\multicolumn{3}{|c|}{\textbf{Normalized Area}}                                                                                                                         & \multicolumn{1}{c|}{1.36}    & 1                                                                     \\ \hline
\end{tabular}
\end{table}

% focus on analog vs digital
% change analog to mixed-signal implementation
% put digital stuff ahead
% observation: analog implementation mainly relieves buffer overhead.
% can observation generalize to other analog implementations?
% add area number and power number? power density?
% add digital version of 0.5/0.8-V paper.

==> table/table_usecase_senputing.tex <==
\begin{table}[t]
%\scriptsize

\centering
\caption{Energy Estimation of Different Analog Implementations For Senputing CIS [pJ/pixel]}
\begin{tabular}{|c|cc|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Analog Compute\\ Position\end{tabular}} & \multicolumn{1}{c|}{Pixel} & Column \\ \hline
\textbf{Technology}                                                        & \multicolumn{2}{c|}{180nm}          \\ \hline
\textbf{Frame Rate}                                                        & \multicolumn{2}{c|}{156fps}         \\ \hline
\textbf{Pixel}                                                             & \multicolumn{1}{c|}{0.24}  & 5.56   \\ \hline
\textbf{SRAM}                                                              & \multicolumn{1}{c|}{1.97}  & 2.62   \\ \hline
\textbf{SCI}                                                               & \multicolumn{1}{c|}{-}     & 30.85  \\ \hline
\end{tabular}
\end{table}

==> table/table_validation_examples_analog.tex <==
\begin{table*}[t]
%\scriptsize

\centering
\caption{Summary of CIS designs used for validation. \fixme{add paper references.}}
\begin{tabular}{|c|c|c|c|ccc|cc|}
\hline
\multirow{2}{*}{} & \multirow{2}{*}{\textbf{Stacked?}} & \multirow{2}{*}{\textbf{Pixel}} & \multirow{2}{*}{\textbf{Analog Memory?}} & \multicolumn{3}{c|}{\textbf{Analog Compuation}}                                                         & \multicolumn{2}{c|}{\textbf{Digital Computation}} \\ \cline{5-9} 
                  &                                  &                                 &                                          & \multicolumn{1}{c|}{\textbf{Type}}           & \multicolumn{1}{c|}{\textbf{Position}} & \textbf{Domain} & \multicolumn{1}{c|}{Type}        &  PE size      \\ \hline
ISSCC'17          &                                  & 3T APS                          & yes, passive and active                  & \multicolumn{1}{c|}{averaging/add}           & \multicolumn{1}{c|}{column/chip}       & charge/voltage         &  \multicolumn{1}{c|}{vector}   &  $4\times4\times64$   \\ \hline
JSSC'19           &                                  & 4T APS                          & yes, active                              & \multicolumn{1}{c|}{logarithmic subtraction} & \multicolumn{1}{c|}{column}            & voltage         & \multicolumn{2}{c|}{N.A.}  \\ \hline
Sensors'20        &                                  & 4T APS                          & no                                       & \multicolumn{1}{c|}{MAC/max-pooling}         & \multicolumn{1}{c|}{column}            & voltage         & \multicolumn{2}{c|}{N.A.}  \\ \hline
ISSCC'21           &                                  & \fixme{??}                            & no                                       & \multicolumn{1}{c|}{\fixme{N.A.?}}                    & \multicolumn{1}{c|}{\fixme{N.A.?}}          & \multicolumn{1}{c|}{\fixme{N.A.?}}     & \multicolumn{1}{c|}{vector}   &  $1\times2304$              \\ \hline
JSSC'21-I           &                                  & PWM                             & no                                       & \multicolumn{1}{c|}{MAC}                     & \multicolumn{1}{c|}{column}            & time/current   & \multicolumn{2}{c|}{N.A.} \\ \hline
JSSC'21-II           &                                  & 4T APS                          & no                                       & \multicolumn{1}{c|}{MAC}                     & \multicolumn{1}{c|}{column}            & charge          & \multicolumn{2}{c|}{N.A.}  \\ \hline
ISSCC'22          &                                  & PWM                             & no                                       & \multicolumn{1}{c|}{MAC}                     & \multicolumn{1}{c|}{column}            & time/current    & \multicolumn{1}{c|}{scalar}            &    $1$            \\ \hline

TCAS-I'22         &                                  & 3T APS                          & no                                       & \multicolumn{1}{c|}{multiply/add}            & \multicolumn{1}{c|}{pixel/chip}        & current         &\multicolumn{2}{c|}{N.A.}      \\ \hline



\end{tabular}
\label{tbl:validation_example}
\end{table*}
